Adaptive Clustering Using Kernel Density Estimators

We derive and analyze a generic, recursive algorithm for estimating all splits in a finite cluster tree as well as the corresponding clusters. We further investigate statistical properties of this generic clustering algorithm when it receives level set estimates from a kernel density estimator. In particular, we derive finite sample guarantees, consistency, rates of convergence, and an adaptive data-driven strategy for choosing the kernel bandwidth. For these results we do not need continuity assumptions on the density such as H\"{o}lder continuity, but only require intuitive geometric assumptions of non-parametric nature.

==> inclusion.tex <==
\section{Uncertainty Control}\label{sec:uq}




% For now, we assume that our kernel is of the form 
% \begin{align}\label{stump-kernel}
%    K(z)=\eins_{[0,1]}\bigl(\snorm z\bigr)\, , \qquad z\in \R^d.
% \end{align}
% where $\snorm\cdot$ is a norm on $\R^d$. For ease of notation, we additionally assume that 
% $\mu$ is a rescaled verison of the Lebesgue measure satisfying $\mu(B_{\snorm\cdot})=1$,
% where $B_{\snorm\cdot}$ denotes the unit ball with respect to the norm $\snorm\cdot$.



% To quantify horizontal uncertainty, we need, for 
% $A\subset X$,
% $\d>0$, the sets
% \begin{align*}
%    A\pde &:= \{x\in X: d(x,A) \leq \d\}\, ,\\
%    A\mde &:= X\setminus (X\setminus A)\pde\, ,
% \end{align*}
% where $d(x,A) := \inf_{x'\in A}\snorm{x -x'}$ denotes the distance between $x$ and $A$.



% \begin{theorem}\label{include-main-thm}
% Let $K:\R^d\to \R$ be a kernel of the form \eqref{stump-kernel} and  
% $P$
% be a $\mu$-absolutely continuous probability measure on $\R^d$ that is normal at every level, and $D\in X^n$ be a 
% data set such that  $\inorm{\hdd-\hpd}<\varepsilon$ for some $\varepsilon>0$ and $\d>0$.
% For $\r\geq 0$ we define 
% \begin{align}\label{Lrho}
%    L_{D,\r} := \{x\in D:\hdd(x) \geq \r\}\pde
% \end{align}
% Then, for all  $\rho\ge 0$, we have
% \begin{align}\label{connect-main}
%    M\mtde_{\r+\e} \subset L_{D,\r} \subset  M\ptde_{\r-\e}\, .
% \end{align}
% \end{theorem}

% In the following, we call a function  $K:\R^d\to [0,\infty)$ with 
% $\int_{\R^d} Kd\mu = 1$ and
% $K(x) = K(-x)$ for all $x\in \Rd$
% a symmetric kernel. For $\d>0$ we further write $K_\d := \d^{-d} K(\d^{-1}\, \cdot\,)$. 
% For later use we note that this yields
% \begin{equation}\label{shift-inv-supp}
%    \supp K_\d(x-\cdot)\subset B(x,\delta)
% \end{equation}
% and 
% \begin{equation}\label{shift-int-kernel}
%      \int_{\Rd}K_\d\Bigl(\frac{x-y}\d  \Bigr) \,d\mu(y) = \int_{\Rd}K ({x-y}) \,d\mu(y)  = \int_{\Rd}K ({y-x}) \,d\mu(y)= 1
% \end{equation}
% for all $x\in \Rd$, $\d>0$.

% \begin{theorem}\label{include-main-thm-new}
% Let $K:\R^d\to [0,\infty)$ be a symmetric kernel with $\supp K\subset B_{\snorm\cdot}$.
% Moreover, let
% $P$
% be a $\lbd$-absolutely continuous probability measure on $\R^d$ that is normal at every level, and $D\in X^n$ be a 
% data set such that the corresponding KDE satisfies $\inorm{\hdd-\hpd}<\varepsilon$ for some $\varepsilon>0$ and $\d>0$.
% For $\r\geq 0$ we define 
% \begin{align}\label{Lrho}
%    L_{D,\r} := \{x\in D:\hdd(x) \geq \r\}\pde
% \end{align}
% Then, for all  $\rho\ge 0$, we have
% \begin{align}\label{connect-main}
%    M\mtde_{\r+\e} \subset L_{D,\r} \subset  M\ptde_{\r-\e}\, .
% \end{align}
% \end{theorem}



